Exploring the mass and redshift dependence of the cluster pressure profile with stacks on thermal SZ maps

We provide novel constraints on the parameters defining the universal pressure profile (UPP) within clusters of galaxies, and explore their dependence on the cluster mass and redshift, from measurements of Sunyaev-Zel'dovich Compton-$y$ profiles. We employ both the $\textit{Planck}$ 2015 MILCA and the ACT-DR4 $y$ maps over the common $\sim 2,100\,\text{deg}^2$ footprint. We combine existing cluster catalogs based on KiDS, SDSS and DESI observations, for a total of 23,820 clusters spanning the mass range $10^{14.0}\,\text{M}_{\odot}<M_{500}<10^{15.1}\,\text{M}_{\odot}$ and the redshift range $0.02<z<0.98$. We split the clusters into three independent bins in mass and redshift; for each combination we detect the stacked SZ cluster signal and extract the mean $y$ angular profile. The latter is predicted theoretically adopting a halo model framework, and MCMCs are employed to estimate the UPP parameters, the hydrostatic mass bias $b_{\rm h}$ and possible cluster miscentering effects. We constrain $[P_0,c_{500},\alpha,\beta]$ to $[5.9,2.0,1.8,4.9]$ with $\textit{Planck}$ and to $[3.8,1.3,1.0,4.4]$ with ACT using the full cluster sample, in agreement with previous findings. We do not find any compelling evidence for a residual mass or redshift dependence, thus expanding the validity of the cluster pressure profile over much larger $M_{500}$ and $z$ ranges; this is the first time the model has been tested on such a large (complete and representative) cluster sample. Finally, we obtain loose constraints on the hydrostatic mass bias in the range 0.2-0.3, again in broad agreement with previous works.

==> tables/cmptable.tex <==
\begin{table*}
\centering
\caption{Numbers.}
\label{tab:stats}
\setlength{\tabcolsep}{1.2em}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{c|c|cccc}
\hline
 & \diagbox[width=10em]{z}{$M_{500}$} & $[10^{13.8},10^{14.2}] \,\text{M}_{\odot}$ & $[10^{14.2},10^{14.6}] \,\text{M}_{\odot}$ & $[10^{14.6},10^{15.2}] \,\text{M}_{\odot}$ & All $M_{500}$\\
\hline
 $\mathbf{N_{\textbf{sc}}}$ & \multirow{2}{8em}{$[0.00,0.35]$} & \color{red}{5458} & \color{red}{1507} & \color{red}{335} & \color{red}{7300} \\  $\mathbf{N_{\textbf{or}}}$ &  & \color{blue}{6296} & \color{blue}{2784} & \color{blue}{672} & \color{blue}{9752} \\ 
\hline
 $\mathbf{N_{\textbf{sc}}}$ & \multirow{2}{8em}{$[0.35,0.70]$} & \color{red}{15622} & \color{red}{4554} & \color{red}{1056} & \color{red}{21232} \\  $\mathbf{N_{\textbf{or}}}$ &  & \color{blue}{14681} & \color{blue}{9017} & \color{blue}{1567} & \color{blue}{25265} \\ 
\hline
 $\mathbf{N_{\textbf{sc}}}$ & \multirow{2}{8em}{$[0.70,1.05]$} & \color{red}{3716} & \color{red}{1648} & \color{red}{290} & \color{red}{5654} \\  $\mathbf{N_{\textbf{or}}}$ &  & \color{blue}{3872} & \color{blue}{1511} & \color{blue}{287} & \color{blue}{5670} \\ 
\hline
 $\mathbf{N_{\textbf{sc}}}$ & \multirow{2}{8em}{All $z$} & \color{red}{24796} & \color{red}{7709} & \color{red}{1681} & \color{red}{34186} \\  $\mathbf{N_{\textbf{or}}}$ &  & \color{blue}{24849} & \color{blue}{13312} & \color{blue}{2526} & \color{blue}{40687} \\ 
\hline
\end{tabular}
\end{table*}


==> tables/linear_regression.tex <==
\begin{table}
\centering
	\caption{Best-fit parameters for the linear regression employed to scale WHL and DESI masses to the retrieved KiDS matches, according to equation~\eqref{eq:linfit}.}
\label{tab:regression}
\renewcommand{\arraystretch}{1.5}
\begin{tabular}{M{0.2cm}|M{1.7cm}M{1.7cm}M{1.7cm}M{1.7cm}}
\hline
\multicolumn{5}{c}{WHL}  \\
\hline
$z$ & $[0.00,0.35]$ & $[0.35,0.45]$ & $[0.45,0.55]$ & $[0.55,0.80]$ \\
$m$  & $1.04\pm0.08$  & $1.06\pm0.08$  & $1.05\pm0.09$  & $1.08\pm0.11$  \\
$q$  & $-0.09\pm0.03$  & $-0.04\pm0.03$  & $-0.06\pm0.03$  & $-0.07\pm0.03$  \\
\hline
\multicolumn{5}{c}{DESI}  \\
\hline
$z$ & $[0.00,0.35]$ & $[0.35,0.45]$ & $[0.45,0.55]$ & $[0.55,0.80]$ \\
$m$  & $0.86\pm0.08$  & $0.82\pm0.07$  & $1.10\pm0.08$  & $0.95\pm0.06$  \\
$q$  & $0.01\pm0.03$  & $0.05\pm0.02$  & $-0.02\pm0.02$  & $0.03\pm0.02$  \\
\end{tabular}
\end{table}

